aspcud: A Linux Package Configuration Tool Based on Answer Set Programming

We present the Linux package configuration tool aspcud based on Answer Set Programming. In particular, we detail aspcud's preprocessor turning a CUDF specification into a set of logical facts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{C. Drescher, I. Lynce and R. Treinen (eds.):\\ Workshop on Logics for Component Configuration (LoCoCo 2011)\\
EPTCS 65, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.65.2}{10.4204/EPTCS.65.2}}
\pdfoutput=1

